Leveraging LLMs for Unsupervised Dense Retriever Ranking

In this paper we present Large Language Model Assisted Retrieval Model Ranking (LARMOR), an effective unsupervised approach that leverages LLMs for selecting which dense retriever to use on a test corpus (target). Dense retriever selection is crucial for many IR applications that rely on using dense retrievers trained on public corpora to encode or search a new, private target corpus. This is because when confronted with domain shift, where the downstream corpora, domains, or tasks of the target corpus differ from the domain/task the dense retriever was trained on, its performance often drops. Furthermore, when the target corpus is unlabeled, e.g., in a zero-shot scenario, the direct evaluation of the model on the target corpus becomes unfeasible. Unsupervised selection of the most effective pre-trained dense retriever becomes then a crucial challenge. Current methods for dense retriever selection are insufficient in handling scenarios with domain shift. Our proposed solution leverages LLMs to generate pseudo-relevant queries, labels and reference lists based on a set of documents sampled from the target corpus. Dense retrievers are then ranked based on their effectiveness on these generated pseudo-relevant signals. Notably, our method is the first approach that relies solely on the target corpus, eliminating the need for both training corpora and test labels. To evaluate the effectiveness of our method, we construct a large pool of state-of-the-art dense retrievers. The proposed approach outperforms existing baselines with respect to both dense retriever selection and ranking. We make our code and results publicly available at https://github.com/ielab/larmor/.

==> Sections/outlook.tex <==
\section{Outlook}

We have examined the effectiveness of adapting methods of unsupervised performance evaluation with the presence of domain shift, proposed in the area of computer vision and machine learning, to the problem of choosing which dense retriever model to use when searching on a new collection for which no labels are available, i.e. in a zero-shot setting.

Our first finding is that the in-domain effectiveness of the dense retrievers, trained on a large corpus like MS MARCO, represents a strong indicator of model generalizability on the target domains, despite the existence of domain gap. 
However, we note that the problem of dense retrieval selection, i.e. which dense retriever model to select in a new domain, remains an important and unresolved issue. Specifically, we observe that the straightforward in-domain-based model selection method fails to choose the best model across all the datasets examined. Furthermore, for certain datasets, the ranking of models based on this method is significantly flawed. The methods we have investigated and that we have adapted from computer vision and machine learning can only do as well as this simple baseline (though some do notably worse).
These findings highlight the need for further research to improve the effectiveness of model selection techniques to make feasible the practical application of dense retrieval in domain-specific tasks characterized by low labeled data availability.

In this work, we focus on a realistic model selection scenario in information retrieval, which differs from the artificially-created setups investigated in prior work in machine learning (see Challenge 1 in Section~\ref{subsection:challenges}). Due to the challenges in adapting model selection methods to the information retrieval setup, we primarily considered two broad groups of methods: uncertainty-based and activation-based. 

\textbf{Uncertainty-based methods.} In the field of machine learning, entropy-based methods are often used to measure the level of uncertainty of a model. These methods analyze the score distribution produced by the model and use it to assess the model's level of confidence in its predictions.

In classification tasks, the concept of uncertainty is naturally linked to the score distribution since there is only one correct class per input sample. When a model predicts two classes with similar probabilities, it indicates uncertainty about the sample's classification.

In information retrieval tasks, the requirement for an ideal ranker is to maximize the binary entropy of relevant document predictions and minimize the binary entropy of irrelevant ones, as defined by~\citet{10.1145/1076034.1076042}. This presents a challenge since the number of relevant documents in an unjudged collection is unknown. As a result, the connection between score distribution and model uncertainty in ranking tasks is not intuitive. 
For instance, a retriever that produces a steep score distribution with a top-ranked document having a significantly higher score than other retrieved documents will have a small entropy score. On the other hand, a retriever with a more gradually-declining score distribution will have a larger entropy score. However, having a large entropy of predictions does not necessarily imply that the model is uncertain. It may instead reflect that the model predicts more the top-k retrieved documents to be equally relevant. In addition, the nature of the dataset itself could highly influence the score distributions. Large datasets with many documents that are relevant to a query will likely result in rankings with low entropy; while small datasets with very different documents and with just a handful of documents that are close to the query will likely result in rankings with a high entropy. In this example, however, the case with higher entropy does not indicate the model is more certain about its predictions.

%  In fact, based on the nature of the datasets, the desired  for the entropy might vary: for    

Another way to define the uncertainty of the model is to evaluate its robustness to query perturbation. The intuition is that if the model is confident in its predictions, it should not be affected by a slight perturbation of the query. Consequently, network robustness can be used as a quality measure of the model, and employed as an unsupervised criterion for model selection. Indeed, according to our results, this approach provides competitive model ranking, with an average Tau Correlation of -0.189. Despite this, the correlation is very weak and the method falls noticeably behind the top-performing baseline, indicating that there is still ample opportunity for improvement, which we recommend the information retrieval community should explore in future research.    


% Rephrase it!
%Uncertainty estimation in information retrieval is an essential yet relatively unexplored problem~\cite{turtle1997uncertainty,crestani1998information,collins2007estimation}, particularly for rankers based on pre-trained language models. Recent attempts have been made to model uncertainty for neural rankers such as the Transformer Pointer Generator Network (T-PGN) model~\cite{lesota2021modern}, or Cohen et al.'s~\cite{cohen2021not} efficient uncertainty and calibration modeling based on Monte-Carlo drop-out~\cite{gal2016dropoutal}. More effective and meaningful estimations of uncertainty might be a promising future direction.
%
%
%
%Uncertainty estimation in Information Retrieval is a fundamental yet largely unexplored problem~\cite{turtle1997uncertainty,crestani1998information,collins2007estimation}, especially for rankers based on PLMS~\cite{lesota2021modern,cohen2021not}. Attempts have been made to exploit uncertainty in relevance estimation for traditional statistical models such as language models and BM25~\cite{zhu2009risky,wang2009portfolio}, but in these works the actual estimation of uncertainty is based on assumptions and heuristics such as to be related to similarities or covariance between term occurrences~\cite{zhu2009risky,wang2009portfolio,zuccon2009quantum}, to follow the Dirichlet distribution~\cite{wang2009portfolio}, or to be computed based on score distributions obtained through query term resampling~\cite{collins2007estimation}. Recent attempts have been made to model uncertainty for neural rankers, for example Transformer Pointer Generator Network (T-PGN) model~\cite{lesota2021modern}, or Cohen et al.'s~\cite{cohen2021not} efficient uncertainty and calibration modelling strategies based on Monte-Carlo drop-out~\cite{gal2016dropoutal}, but these are not readily applicable to the PLM ranker architectures we consider. In future work we plan to adapt and investigate these uncertainty estimations.


The issue of uncertainty estimation in information retrieval is a significant yet largely under-explored problem, as noted in several prior studies~\cite{turtle1997uncertainty, crestani1998information, collins2007estimation}. This is particularly true for rankers that rely on pre-trained language models~\cite{lesota2021modern}. While some efforts have been made to leverage uncertainty in relevance estimation for traditional keyword-based best-match models like BM25 and language models, the current approaches are based on assumptions and heuristics that use similarities or covariance between term occurrences~\cite{zhu2009risky, wang2009portfolio, zuccon2009quantum}, follow the Dirichlet distribution~\cite{wang2009portfolio}, or calculate score distributions by resampling query terms~\cite{collins2007estimation}. Recently, researchers have attempted to model uncertainty for neural rankers, such as the Transformer Pointer Generator Network (T-PGN) model~\cite{lesota2021modern} 
%or Cohen et al.'s~\cite{cohen2021not} efficient uncertainty and calibration modeling techniques that rely on Monte-Carlo drop-out~\cite{gal2016dropout}. 
However, these models are not easily adaptable to the dense retrieval ranker architectures that we have examined in this paper. More effective and meaningful estimations of uncertainty might be a promising future direction also in our context.



\textbf{Activation-based methods.}
Activation-based methods approximate the domain gap between the source and target distributions via the proximity of its hidden representations. The underlying idea is that a model with good generalization capabilities should produce similar encodings for both datasets.
The advantage of this method if adapted to information retrieval is that it is not affected by variations in network architectures or scoring functions used, which enables the comparison of models within the constraints of the information retrieval setup (i.e. across different pre-trained language models and architectures). This makes it easier to identify models that perform well on both source and target datasets, without being biased towards specific network architectures or scoring functions. 

In our experiments, we used the Fréchet distance between the activations of the network for the source and target datasets (Method 3, Corpus Similarity).  This approach, highly effective for example in computer vision tasks, in our experiments selects the same best model for all the datasets, similarly to the in-domain performance-based method, but produces an inferior model ranking (see Table \ref*{tab:tau_ndcg@10}). To handle the high dimensionality of the activation spaces, the Fréchet-based approximation assumes that they conform to a normal distribution~\cite{Chong2019EffectivelyUF}, which may not hold for NLP-induced hidden representations. We believe that designing NLP-oriented distance approximations between activation spaces is a promising future direction for more accurate unsupervised model selection, especially in the context of selecting dense retrieval models.  

\textbf{Weight- and Performance-based methods.} The last direction we would like to mention is inspired the recent work by \citet{khramtsova} and \citet{Deng2021WhatDR} which involves fine-tuning the network on the target dataset with the unsupervised loss (e.g., it can be a masked token prediction task) and evaluating the degree of the network change or the performance on the unsupervised task. Despite being computationally expensive, these approaches have been shown very effective in general machine learning model selection, and can be further explored in the information retrieval context.


==> Sections/result_extra.tex <==


%($\downarrow$)
\begin{table*}[t]
    \caption{$\Delta_e$, calculated based on recall@1000. \vspace{-10pt}}
\resizebox{\textwidth}{!}{
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
        
        
        \hline
        &  NF & FiQA & ArguAna & SciDocs & SciFact& Covid & Quora&  NQ & DBPedia & HotpotQA  & Signal1M & Robust04 & Trec-News &\textbf{Avrg}\\
        % \hline
        % \texttt{MSMARCO Perf.} & 6.84 & 20.21 & 27.47 & 10.02 & 20.26 & 32.18 & 9.58 & 13.91 & 9.80 & 17.52 & 3.51 & 20.23 & 16.89 & 16.03\\
        \texttt{Binary Entropy} &7.91 & 12.13 & 0.35 & 35.09 & 4.33 & 8.02 & 0.04 & 16.13 & 13.29 & 27.28 & 17.65 & 8.19 & 20.8 & 13.17 \\        \hline
        \texttt{Query Alteration} &3.31 & 10.8 & 0.0 & 17.38 & 2.67 & 6.52 & 0.07 & 2.19 & 6.79 & 14.66 & 16.39 & 8.19 & 5.47 & 7.26 \\
        \texttt{WIG} & 12.99 & 20.96 & 0.28 & 31.81 & 4.17 & 32.79 & 0.36 & 5.66 & 22.27 & 24.7 & 18.37 & 25.18 & 24.8 & 17.26\\
        \texttt{WIG Norm} &  13.41 & 15.97 & 0.64 & 35.09 & 4.33 & 18.79 & 0.16 & 6.35 & 31.82 & 27.29 & 18.06 & 20.71 & 20.8 & 16.42 \\        
        \texttt{NQC} & 12.44 & 5.52 & 0.14 & 3.92 & 0.33 & 32.79 & 0.13 & 1.5 & 14.83 & 21.38 & 3.27 & 25.18 & 12.67 & 10.32\\ 
        \texttt{NQC Norm} & 12.99 & 20.96 & 0.28 & 31.81 & 4.17 & 32.79 & 0.36 & 5.66 & 22.27 & 24.7 & 18.37 & 25.18 & 24.8 &  17.26\\        
        \texttt{SMV} & 12.44 & 5.52 & 0.14 & 3.92 & 0.33 & 32.79 & 0.06 & 1.5 & 14.83 & 28.24 & 3.27 & 25.18 & 12.67 & 10.84 \\
        \texttt{SMV Norm} & 12.99 & 20.96 & 0.28 & 31.81 & 4.17 & 32.79 & 0.36 & 5.66 & 22.27 & 24.7 & 18.37 & 25.18 & 24.8 & 17.26 \\
        
        $\sigma$ & 12.99 & 20.96 & 0.28 & 31.81 & 4.17 & 32.79 & 0.36 & 5.66 & 22.27 & 24.7 & 18.37 & 25.18 & 24.8 & 17.26 \\
        $\sigma_{max}$ & 12.99 & 20.96 & 0.28 & 31.81 & 4.17 & 32.79 & 0.36 & 5.66 & 22.27 & 24.7 & 18.37 & 25.18 & 24.8 &  17.26\\
        \texttt{Clarity} & 1.68 & 8.2 & 0.0 & 4.48 & 2.33 & 10.55 & 0.06 & 0.46 & 12.9 & 21.98 & 13.45 & 25.18 & 14.58 & 8.91 \\
        \texttt{Fusion} &0.78 & 2.75 & 0.0 & 13.72 & 0.33 & 8.17 & 0.01 & 0.05 & 2.43 & 4.63 & 3.5 & 0.07 & 0.0 & 2.8 \\        % flan-t5-xl-q10.fusion-top100
        %Eval Judg & 1.52 & 3.07 & 0.59 & 3.26 & 2.01 & 18.29 & 0.0 & 0.58 & 0.82 & 1.21 & 1.7 & 9.36 & 0.0 & 3.26 \\ 
        % flan-t5-xl-q10.fusion-setwise
        %Eval RBO &  0.22 & 5.46 & 7.96 & 3.9 & 1.48 & 20.09 & 0.94 & 9.29 & 2.53 & 7.17 & 0.25 & 2.37 & 0.0 & 4.74 \\ 
        % rank_flan-t5-xl-q10.fusion-top100-fusion-setwise-fusion-rrf
        LARMOR T5-xl Q & 2.85 & 2.75 & 0.07 & 10.08 & 0.0 & 10.32 & 0.0 & 0.0 & 7.71 & 2.3 & 10.38 & 8.11 & 5.47 & 4.62 \\
        
        % gpt-3.5-turbo-1106 & 1.52 & 12.76 & 0.0 & 3.9 & 2.01 & 20.74 & 3.41 & 12.3 & 3.6 & 1.74 & 4.24 & 7.92 & 9.56 & 6.44 \\
        % gpt-4-1106-preview & 1.52 & 12.76 & 0.0 & 3.62 & 0.77 & 18.31 & 3.41 & 0.58 & 9.87 & 5.74 & 4.24 & 2.37 & 4.68 & 5.22\\
        % flan-t5-xl & 1.52 & 5.46 & 13.73 & 3.26 & 2.01 & 18.29 & 0.0 & 0.58 & 3.87 & 3.1 & 1.38 & 7.92 & 5.95 &  5.16 \\
        \hline
        
        \hline
    \end{tabular}
}
\vspace{-6pt}
\label{tab:delta}
\end{table*}









\begin{table*}[t]
    \caption{$\Delta_e$, calculated based on MAP@1000. \vspace{-10pt}}
\resizebox{\textwidth}{!}{
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
        
        
        \hline
        &  NF & FiQA & ArguAna & SciDocs & SciFact& Covid & Quora&  NQ & DBPedia & HotpotQA  & Signal1M & Robust04 & Trec-News &\textbf{Avrg}\\
        % \hline
        % \texttt{MSMARCO Perf.} & 6.84 & 20.21 & 27.47 & 10.02 & 20.26 & 32.18 & 9.58 & 13.91 & 9.80 & 17.52 & 3.51 & 20.23 & 16.89 & 16.03\\
        \texttt{Binary Entropy} &6.14 & 16.97 & 25.53 & 9.35 & 24.77 & \textbf{7.58} & 2.59 & 31.82 & 7.05 & 30.04 & 5.52 & 6.45 & 14.69 & 14.5 \\    
        \texttt{Query Alteration} &2.17 & 14.64 & \textbf{8.44} & 5.16 & 18.3 & \textbf{7.18} & 4.2 & 20.73 & 2.81 & 21.48 & 4.09 & 6.45 & 7.42 & 9.47 \\
        \texttt{WIG} & 9.35 & 25.78 & 22.28 & 9.99 & 26.31 & 26.64 & 8.49 & 26.62 & 15.71 & 32.5 & 5.77 & 14.41 & 20.12 & 18.77\\       
        \texttt{WIG Norm} &  10.27 & 18.96 & 23.02 & 9.35 & 24.78 & 15.19 & 4.52 & 18.72 & 17.18 & 30.04 & 3.72 & 11.79 & 14.69 & 15.55 \\        
        \texttt{NQC} & 9.37 & 12.16 & 15.28 & 1.44 & 10.51 & 26.64 & 4.17 & 17.73 & 10.72 & 24.18 & 1.87 & 14.41 & 10.13 & 12.2\\ 
        \texttt{NQC Norm} & 9.35 & 25.78 & 22.28 & 9.99 & 26.31 & 26.64 & 8.49 & 26.62 & 15.71 & 32.5 & 5.77 & 14.41 & 20.12 & 18.77\\        
        \texttt{SMV} & 9.37 & 12.16 & 15.28 & 1.44 & 10.51 & 26.64 & 4.29 & 17.73 & 10.72 & 29.68 & 1.87 & 14.41 & 10.13 & 12.63\\
        \texttt{SMV Norm} & 9.35 & 25.78 & 22.28 & 9.99 & 26.31 & 26.64 & 8.49 & 26.62 & 15.71 & 32.5 & 5.77 & 14.41 & 20.12 &18.77\\       
        $\sigma$ & 9.35 & 25.78 & 22.28 & 9.99 & 26.31 & 26.64 & 8.49 & 26.62 & 15.71 & 32.5 & 5.77 & 14.41 & 20.12 & 18.77\\
        $\sigma_{max}$ & 9.35 & 25.78 & 22.28 & 9.99 & 26.31 & 26.64 & 8.49 & 26.62 & 15.71 & 32.5 & 5.77 & 14.41 & 20.12 & 18.77 \\
        \texttt{Clarity} & 2.06 & 11.61 & 18.53 & 1.64 & 12.57 & 11.27 & 3.95 & 3.99 & 12.09 & 34.97 & 1.9 & 14.41 & 7.91 & 10.53 \\
       
        \texttt{Fusion} &\textbf{1.17} & 4.59 & 8.56 & 4.41 & 4.19 & 8.82 & 1.13 & 9.82 & 1.89 & 7.84 & 1.25 & 0.17 & \textbf{0.0} & 4.14\\        % flan-t5-xl-q10.fusion-top100
        %Eval Judg & 1.52 & 3.07 & 0.59 & 3.26 & 2.01 & 18.29 & 0.0 & 0.58 & 0.82 & 1.21 & 1.7 & 9.36 & 0.0 & 3.26 \\ 
        % flan-t5-xl-q10.fusion-setwise
        %Eval RBO &  0.22 & 5.46 & 7.96 & 3.9 & 1.48 & 20.09 & 0.94 & 9.29 & 2.53 & 7.17 & 0.25 & 2.37 & 0.0 & 4.74 \\ 
        % rank_flan-t5-xl-q10.fusion-top100-fusion-setwise-fusion-rrf
        LARMOR T5-xl Q & 2.02 & 4.59 & 13.81 & 2.8 & 1.91 & 9.42 & \textbf{0.0} & 0.79 & 4.09 & 3.42 & 1.82 & 4.96 & 7.42 & 4.39 \\
        % gpt-3.5-turbo-1106 & 1.52 & 12.76 & 0.0 & 3.9 & 2.01 & 20.74 & 3.41 & 12.3 & 3.6 & 1.74 & 4.24 & 7.92 & 9.56 & 6.44 \\
        % gpt-4-1106-preview & 1.52 & 12.76 & 0.0 & 3.62 & 0.77 & 18.31 & 3.41 & 0.58 & 9.87 & 5.74 & 4.24 & 2.37 & 4.68 & 5.22\\
        % flan-t5-xl & 1.52 & 5.46 & 13.73 & 3.26 & 2.01 & 18.29 & 0.0 & 0.58 & 3.87 & 3.1 & 1.38 & 7.92 & 5.95 &  5.16 \\
        \hline
        
        \hline
    \end{tabular}
}
\vspace{-6pt}
\label{tab:delta}
\end{table*}

